Diffuse, Attend, and Segment: Unsupervised Zero-Shot Segmentation using Stable Diffusion

Producing quality segmentation masks for images is a fundamental problem in computer vision. Recent research has explored large-scale supervised training to enable zero-shot segmentation on virtually any image style and unsupervised training to enable segmentation without dense annotations. However, constructing a model capable of segmenting anything in a zero-shot manner without any annotations is still challenging. In this paper, we propose to utilize the self-attention layers in stable diffusion models to achieve this goal because the pre-trained stable diffusion model has learned inherent concepts of objects within its attention layers. Specifically, we introduce a simple yet effective iterative merging process based on measuring KL divergence among attention maps to merge them into valid segmentation masks. The proposed method does not require any training or language dependency to extract quality segmentation for any images. On COCO-Stuff-27, our method surpasses the prior unsupervised zero-shot SOTA method by an absolute 26% in pixel accuracy and 17% in mean IoU. The project page is at \url{https://sites.google.com/view/diffseg/home}.

==> figures/aggregation_merging.tex <==
\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/aggregation.png}
         % \caption{Attention Aggregation}
         \label{fig:aggregation}
     \end{subfigure}
     % \hfill
     % \begin{subfigure}[b]{0.5\textwidth}
     %     \centering
     %     \includegraphics[width=\textwidth]{figures/merging.png}
     %     \caption{Iterative Attention Merging}
     %     \label{fig:merging}
     % \end{subfigure}
        \caption{Visualization of Attention Aggregation/ An Attention map from a lower resolution is first upsampled and then added to several corresponding higher-resolution maps.}
\end{figure}


==> figures/comparisons.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/comparisons_pdf.pdf}
    \caption{Qualitative Comparisons with unsupervised clustering algorithms.}
    \label{fig:comparisons}
    \vspace{-5mm}
\end{figure}

==> figures/granularity.tex <==

\begin{figure}[ht]
    \centering
    \vspace{-2mm}
    \includegraphics[width=0.45\textwidth]{figures/granularity_pdf.pdf}\vspace{-3mm}
    \caption{Segmentation with different KL threshold $\tau$. $\tau$ controls the granularity. Controllability is a trait of DiffSeg.}
    \label{fig:granularity}
    \vspace{-2mm}
\end{figure}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tables/coco.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|ccc|cc}
    \toprule   
     & \multicolumn{3}{c|}{Requirements} & \multicolumn{2}{c}{Metrics}\\
    \midrule
     Model& LD  & AX & UA & ACC. & mIoU \\
     \midrule
     IIC~\cite{ji2019invariant} & \xmark & \xmark& \cmark & 21.8 & 6.7\\
     MDC~\cite{caron2018deep} & \xmark & \xmark& \cmark & 32.3 & 9.8\\
     PiCLE~\cite{cho2021picie} & \xmark & \xmark& \cmark & 48.1 & 13.8\\
    PiCLE+H~\cite{cho2021picie} & \xmark & \xmark& \cmark & 50.0 & 14.4\\
    STEGO~\cite{hamilton2022unsupervised} & \xmark & \xmark& \cmark & 56.9 & 28.2\\
    ACSeg~\cite{li2023acseg} & \cmark & \xmark& \cmark & - & 28.1\\
    \midrule
    MaskCLIP~\cite{zhou2022extract}& \cmark & \xmark & \xmark& 32.2 & 19.6\\
    ReCo~\cite{shin2022reco}& \cmark & \cmark & \xmark & 46.1 & 26.3\\
    \midrule
    Ours: DiffSeg (320) & \xmark & \xmark& \xmark &  \textbf{72.5} & 43.0\\
    Ours: DiffSeg (512) & \xmark & \xmark& \xmark &  \textbf{72.5} & \textbf{43.6}\\
    \bottomrule
    \end{tabular}
    \caption{Evaluation on COCO-Stuff-27. Language Dependency (LD), Auxiliary Images (AX), Unsupervised Adaptation (UA).}
    \label{tab:coco}
\end{table}

==> tables/rebuttal.tex <==
\begin{table}[ht]
    \centering
    \resizebox{.45\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
          Metrics & K-Means-C & DBSCAN & DiffSeg (Inner) & DiffSeg (0.9) &  DiffSeg (DINO) &DiffSeg\\
          \midrule
          ACC& 58.9 & 57.7 & 62.3& 68.8 & 68.2&\textbf{72.5} \\
          mIoU  & 33.7 & 27.2 & 31.9 &40.2 & 39.1&\textbf{43.6}\\
    \bottomrule
    \end{tabular}}
    \caption{COCO Results with unsupervised clustering algorithm (K-Means, DBSCAN), DiffSeg using the inner product, DiffSeg with 0.9 KL threshold, and DiffSeg with Dino backbone.}
    \label{tab:rebutall}
    \vspace{-5mm}
\end{table}
